Pathways to Leverage Transcompiler based Data Augmentation for Cross-Language Clone Detection

Software clones are often introduced when developers reuse code fragments to implement similar functionalities in the same or different software systems. Many high-performing clone detection tools today are based on deep learning techniques and are mostly used for detecting clones written in the same programming language, whereas clone detection tools for detecting cross-language clones are also emerging rapidly. The popularity of deep learning-based clone detection tools creates an opportunity to investigate how known strategies that boost the performances of deep learning models could be further leveraged to improve clone detection tools. In this paper, we investigate such a strategy, data augmentation, which has not yet been explored for cross-language clone detection as opposed to single-language clone detection. We show how the existing knowledge on transcompilers (source-to-source translators) can be used for data augmentation to boost the performance of cross-language clone detection models, as well as to adapt single-language clone detection models to create cross-language clone detection pipelines. To demonstrate the performance boost for cross-language clone detection through data augmentation, we exploit Transcoder, which is a pre-trained source-to-source translator. To show how to extend single-language models for cross-language clone detection, we extend a popular single-language model, Graph Matching Network (GMN) in a combination with the transcompilers. We evaluated our models on popular benchmark datasets. Our experimental results showed improvements in F1 scores (sometimes up to 3%) for the cutting-edge cross-language clone detection models. Even when extending GMN for cross-language clone detection, the models built leveraging data augmentation outperformed the baseline with scores of 0.90, 0.92, and 0.91 for precision, recall, and F1 score, respectively.

==> notes.tex <==
1. fix parsability issues for GMN input : done
2. R-package for merging phylogenetic tree
3. new dataset, BigCloneBench -transcode-> to get new dataset : done

4. Frequency of token in AST ; this does not change the embedding since two nodes with similar text already have same embedding and with same frequency value it still remains same with another number added.
'int':1 
'k':2

[[1][2]]

frequence 10,
[[1][2]]

%------------------------------------------------------
(edit OR improvement OR modification OR change OR revise OR correction) AND ("stack overflow" OR (Q&A OR question-answer OR developer OR "question and answer" ) AND (site OR website OR forum OR platform))

ACM Digital Library: https://dl.acm.org
Springer: https://link.springer.com
Elsevier: https://www.elsevier.com/solutions/scopus
 IET Digital Library: https://digital-library.theiet.org
World Scientific: https://www.worldscientific.com
Wiley Online Library: https://onlinelibrary.wiley.com
ScienceDirect: https://www.sciencedirect.com
 IEEE Xplore: https://ieeexplore.ieee.org/Xplore/home.jsp
DBLP: https://dblp.uni-trier.de

And sometimes I use the following citation management sites:

1. Connected Papers: https://www.connectedpapers.com

2. Research Rabbit: https://researchrabbitapp.com/home

3. Litmaps: https://app.litmaps.co
**********************
%------------------------------------------------------


For parsable/unparsable:
Convert:
Java->Python
Python->Java'

Java, Java' 

Augment:
J, P
p', j'
Extended pairs
P j'
j p'







**
\and
\IEEEauthorblockN{2\textsuperscript{nd} Debajyoti Mondal}
\IEEEauthorblockA{\textit{Department of Computer Science} \\
\textit{University of Saskatchewan}\\
Saskatoon, Canada \\
d.mondal@usask.ca}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Chanchal K. Roy}
\IEEEauthorblockA{\textit{Department of Computer Science} \\
\textit{University of Saskatchewan}\\
Saskatoon, Canada \\
chanchal.roy@usask.ca}
\and

1. If C4 reproduce -> check data aug -> if improved -then we say Cont 1: DATA aug Cont 2: how to adapt diff DL model
2. If C4 cannot be reproduced -> Chck edge attr ofGMN to beat C4. If cannot beat C4 then contrib is the same as 1 (but what we did is just extra work)

3. If C4 cannot be reproduced -> Chck edge attr ofGMN to beat C4. If can beat C4 then contrib  will be improved significantly


%-----
\begin{table}[htbp]
\caption{Results on Original Dataset}
\begin{center}
\begin{tabular}{l| l c c c c} 
 \hline
 &Model & Precision & Recall & $F_1$ \\
 \hline
\multirow{5}{4em}{ML/DL Models} &Random Forest &0.64 &0.79  &0.71\\
&XGBoost  &0.72 &0.83  &0.77\\
&CLCDSA &0.49(0.46) &0.83(0.85) &0.62(0.60)\\
%CLCDSA* &0.60 & 0.93 & 0.73\\
&C4 &0.94 &90 &0.92\\
&GMN &0.91 &0.92  &0.91\\
\hline
%\multirow{1}{4em}{}
Non-ML Models  &COSAL &0.55 &0.89 &0.68\\
\hline
\end{tabular}
\end{center}
\end{table}

%double pairs augmented
\begin{table}[htbp]
\caption{Results on Augmented Dataset}
\begin{center}
\begin{tabular}{l c c c c} 
 \hline
 Model & Precision & Recall & $F_1$ \\
 \hline 
Random Forest &0.64 &0.79  &0.71\\
XGBoost  &0.72 &0.84  &0.78\\
CLCDSA  &0.54 &0.79 &0.64\\
GMN &0.93 &0.95  &0.94\\
\hline
\end{tabular}
\end{center}
 \end{table}


 
\begin{comment}
    
\setbox0=\hbox{%

\begin{minipage}{\linewidth}
\begin{lstlisting}[columns=flexible,language=Java,numbers=none, style=code_table]

public static int factorial(int n){
    if (n == 0)    
      return 1;    
    else    
        return(n * factorial(n-1));    
 }    
\end{lstlisting}
\end{minipage}
}
\savestack{\listingA}{\box0}

\setbox0=\hbox{%
\begin{minipage}{\linewidth}
\begin{lstlisting}[columns=flexible,language=Python,numbers=none,style=code_table]
def factorial ( n ) :
    if n == 0 : 
        return 1
    else : 
        return (n * factorial(n - 1))
\end{lstlisting}
\end{minipage}
}
\savestack{\listingB}{\box0}
\setbox0=\hbox{%
\begin{minipage}{\linewidth}
\begin{lstlisting}[columns=flexible,language=Java,numbers=none,style=code_table]
public static int factorial(int n){
    if (n == 0)    
      return 1;
      //A comment
    else    
        return(n * factorial(n-1));    
 }    
\end{lstlisting}
\end{minipage}
}
\savestack{\listingC}{\box0}
\begin{figure}[t!]

\stackinset{l}{-5pt}{t}{\llength}{}{\listingA} 
\textbf{(a) Java code for factorial} \\

\stackinset{l}{-5pt}{t}{\llength}{}{\listingB} 
\textbf{(b) Python code by Transcoder}\\

\stackinset{l}{-5pt}{t}{\llength}{}{\listingC} 
\textbf{(c) Java code by  random perturbation}\\

\caption{Example of codes modified differently. The code in (b) is transcompiled through Transcoder from (a), and code in (c) is generated by applying random non-semantic preserving mutation operator.}
\label{fig:example_trans_rand}
\end{figure}



%line plot
\begin{comment}
\begin{tikzpicture}
    \begin{axis}[
        xlabel=$x$,
        ylabel=$y$,
        xmin=0, xmax=30,
        ymin=0, ymax=100,
        xtick={10,20,30},
        ytick={10,20,30,40,50,60,70,80,90,100}
        ]
    \addplot[smooth,mark=*,blue] plot coordinates {
        (0,10)
        (8,30)
        (16,40)
    };
    \addlegendentry{Case 1}

    \end{axis}
    \end{tikzpicture}
\end{comment}

\begin{comment}
\begin{tikzpicture}[x={(.25,0)}]
\foreach  \l/\x/\c[count=\y] in {Original/17.93/original, 
Transcompiled/16.53/trans, 
Mutated/17.8/rand}
{%\node[left] at (0,\y) {\l};
%\draw[fill=\c] (0,\y-.4) rectangle (\x,\y+.4);}
\node[left] at (0,\y) {\l};
\fill[\c] (0,\y-.3) rectangle (\x,\y+.3);
\node[right] at (\x, \y) {\x};}
\draw (0,0) -- (20,0);
\foreach \x in {0, 5, 10, 15, 20}
{\draw (\x,.2) -- (\x,0) node[below] {\x};}
\draw (0,0) -- (0,3.8);
\end{tikzpicture}
\end{comment}
